Valid Post-Detection Inference for Change Points Identified Using Trend Filtering

There are many research works and methods about change point detection in the literature. However, there are only a few that provide inference for such change points after being estimated. This work mainly focuses on a statistical analysis of change points estimated by the PRUTF algorithm, which incorporates trend filtering to determine change points in piecewise polynomial signals. This paper develops a methodology to perform statistical inference, such as computing p-values and constructing confidence intervals in the newly developed post-selection inference framework. Our work concerns both cases of known and unknown error variance. As pointed out in the post-selection inference literature, the length of such confidence intervals are undesirably long. To resolve this shortcoming, we also provide two novel strategies, global post-detection, and local post-detection which are based on the intrinsic properties of change points. We run our proposed methods on real as well as simulated data to evaluate their performances.

==> tex/Sec6_nonsequential_tests_proj2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Inference After Using the Stopping Rule}
\label{sec:nonseq.tests.proj2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section deals with performing statistical inference for change points detected after running the PRUTF algorithm for specific number of steps. Such inference is genuinely different than sequential inference discussed in Sections \ref{sec:post.detection.proj2} and \ref{sec:optimal.conditioning.proj2} which inferential guarantee is carried out across steps of the detection procedure. In other words, at each step of the PRUTF algorithm, the significance of the new estimated change point is evaluated. Instead of testing hypotheses across steps, we could instead make inference for all detected change points after running a certain number of steps of the algorithm. Formally, assume that $\widehat{\bsy\tau}=\{\widehat{\tau}_1,\ldots, \widehat{\tau}_J\}$ is the estimated change points with corresponding signs vector $\widehat{\mbf s}$. The number of steps for the algorithm to gain $\widehat{\bsy\tau}$ can be pre-specified by the user or be chosen adaptively using a criterion which is almost the case in real applications. Therefore, our focus is to compute p-values and construct confidence intervals of $[\mbf D \mbf f]_{\widehat{\tau}_j}$, for $j=1,\ldots, J$. We also assume that the number of steps in the algorithm is derived from the stopping rule presented in Section \ref{sec:stopping.proj2}. Conducting such inferences follows similar logic as that of the sequential case, except conditioning on this adaptively selected number of steps is required. 

We first show that the stopping criterion of \eqref{stop.rule.proj2} also defines a polyhedron constraint for the observations $\mbf y$. Therefore, conditioning the inference on the selected number of step will add a number of rows to the polyhedron matrix $\mbf A$.





















